Guided Feature Selection for Deep Visual Odometry

We present a novel end-to-end visual odometry architecture with guided feature selection based on deep convolutional recurrent neural networks. Different from current monocular visual odometry methods, our approach is established on the intuition that features contribute discriminately to different motion patterns. Specifically, we propose a dual-branch recurrent network to learn the rotation and translation separately by leveraging current Convolutional Neural Network (CNN) for feature representation and Recurrent Neural Network (RNN) for image sequence reasoning. To enhance the ability of feature selection, we further introduce an effective context-aware guidance mechanism to force each branch to distill related information for specific motion pattern explicitly. Experiments demonstrate that on the prevalent KITTI and ICL_NUIM benchmarks, our method outperforms current state-of-the-art model- and learning-based methods for both decoupled and joint camera pose recovery.

==> fig_table/fig_kitti_00_10.tex <==
\begin{figure}[!htb]
	\centering
	\subfigure[BRNN\_lg]{
		\begin{minipage}{0.48\textwidth}
			\centering
			\includegraphics[height=4.cm]{crops/variations/brnn_lg_gt_kitti_10}
			\label{fig:kitti10_a}
	\end{minipage}}
	\vspace{-0.3cm}
	%\hspace{1cm}
	%\qquad
	\subfigure[BRNN\_g]{
		\begin{minipage}{0.48\textwidth}
			\centering
			\includegraphics[height=4.cm]{crops/variations/brnn_g_gt_kitti_10}
			\label{fig:kitti10_b}
	\end{minipage}}
	\subfigure[RNN\_lg]{
		\begin{minipage}{0.48\textwidth}
			\centering
			\includegraphics[height=4.cm]{crops/variations/rnn_lg_gt_kitti_10}
			\label{fig:kitti10_c}
	\end{minipage}}
	%\qquad
	\subfigure[RNN\_g]{
		\begin{minipage}{0.48\textwidth}
			\centering
			\includegraphics[height=4.cm]{crops/variations/rnn_g_gt_kitti_10}
			\label{fig:kitti10_d}
	\end{minipage}}
	\caption{Trajectories of VO results of four variations of our model on KITTI sequence 10.}
	\label{fig:variation_kitti10}
\end{figure}
\setlength{\tabcolsep}{1.4pt}

==> fig_table/table_kitti.tex <==
%We would be glad to respond to further questions and comments you may have.
%\tiny
\setlength{\tabcolsep}{2.4pt}
%\setlength\LTleft{-1in}
%\setlength\LTright{-1in plus 1 fill}
\begin{table}[t]
	\scriptsize
	\centering
		\caption{Results on the KITTI dataset. DeepVO \cite{wang2017deepvo} and our models are trained on Seq 00, 02, 08 and 09, while ESP-VO \cite{wang2017espvo} uses extra Seq 01 in training sets.}
	%\begin{threeparttable}
		\begin{center}
			%\resizebox{\textwidth}{15mm}{
			\begin{tabular}{lclclclclclcl}
				\hline
				\hline
				& \multicolumn{12}{c}{Sequence} \\
				% \cline{2-15} 
				Method & \multicolumn{2}{c}{03} & \multicolumn{2}{c}{04} & \multicolumn{2}{c}{05} & \multicolumn{2}{c}{06} & \multicolumn{2}{c}{07} & \multicolumn{2}{c}{10} \\ 
				%Method & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} &  \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} \\
				& $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$    \\
				\hline
				% DeepVO &  \multicolumn{2}{c} {$- \quad -$} &  \multicolumn{2}{c}{$8.49 \quad 6.89$} &  \multicolumn{2}{c}{$7.19 \quad 6.97$} &  \multicolumn{2}{c}{$2.62 \quad 3.61$} &  \multicolumn{2}{c}{$5.42 \quad 5.82$} &  \multicolumn{2}{c}{$3.91 \quad 4.60$} &  \multicolumn{2}{c}{$8.11 \quad 8.83$} \\
				%ORB\_SLAM-S [5] & 0.71 & 0.18 & 0.48 & 0.13 & 0.40 & 0.16 & 0.51 & 0.15 & 0.50 & 0.28 & 0.60 & 0.27 \\
				%ORB\_SLAM \cite{mur2017orb-slam2} & 0.93 & 0.20 & 0.88 & 0.21 & 12.05 & 0.22 & 19.59 & 0.23 & 13.63 & 0.37 & 24.97 & 0.30 \\
				%ORB\_SLAM-M [5] & 0.93 & 0.20 & 0.88 & 0.21 & 12.05 & 0.22 & 19.59 & 0.23 & 13.63 & 0.37 & 24.97 & 0.30 \\
				VISO2-S \cite{geiger2011stereoscan} & 3.21 & 3.25 & 2.12 & 2.12 & 1.53 & 1.60 & 1.48 & 1.58 & 1.85 & 1.91 & 1.17 & 1.30 \\
				\hline
				VISO2-M \cite{geiger2011stereoscan}   & 8.47 & 8.82 & 4.69 & 4.49 & 19.22 & 17.58 & 7.30 & 6.14 & 23.61 & 19.11 & 41.56 & 32.99 \\
				%ORB\_SLAM \cite{mur2015orb1} & 21.07 & 18.36 & 4.46 & 5.60 & 26.01 & 34.27 & 17.47 & 17.17 & 24.53 & 38.90 & 86.51 & 98.90 \\
				\hline
				\hline
			\end{tabular}
			\label{result_kitti}
			
			%\begin{left}
			\begin{tablenotes}
				%\left
				%\item $*$ORB\_SLAM \cite{mur2017orb-slam2} is not evaluated with other methods since it results are aligned with ground-truth using 7-DoF (rigid body + scale) transformation.
				\footnotesize
				\item $t_{rel}: $ average translational RMSE drift (\%) on length from 100, 200 to 800 m.
				\item $r_{rel}: $ average rotational RMSE drift (${}^{\circ}$/100m) on length from 100, 200 to 800 m.
				%\item Our models and DeepVO are trained on Sequence 00, 02, 08, and 09, while ESP-VO uses additional Sequence 01 for training.
			\end{tablenotes}
		\end{center}
		%\end{left}
	%\end{threeparttable}}
% The best results of monocular VO are highlighted.} %Predicted trajectories of ORB\_SLAM \cite{mur2017orb-slam2} are aligned with ground-truth due to unknown scale. VISO2\_M \cite{geiger2011stereoscan} recovers scale using the fixed camera height as priori.}
	\label{table:table_kitti}
\end{table}
\setlength{\tabcolsep}{1.4pt}
%\setlength{\textfloatsep}{0cm}
